Explainable Predictive Maintenance: A Survey of Current Methods, Challenges and Opportunities

Predictive maintenance is a well studied collection of techniques that aims to prolong the life of a mechanical system by using artificial intelligence and machine learning to predict the optimal time to perform maintenance. The methods allow maintainers of systems and hardware to reduce financial and time costs of upkeep. As these methods are adopted for more serious and potentially life-threatening applications, the human operators need trust the predictive system. This attracts the field of Explainable AI (XAI) to introduce explainability and interpretability into the predictive system. XAI brings methods to the field of predictive maintenance that can amplify trust in the users while maintaining well-performing systems. This survey on explainable predictive maintenance (XPM) discusses and presents the current methods of XAI as applied to predictive maintenance while following the Preferred Reporting Items for Systematic Reviews and Meta-Analyses (PRISMA) 2020 guidelines. We categorize the different XPM methods into groups that follow the XAI literature. Additionally, we include current challenges and a discussion on future research directions in XPM.

==> SECTIONS/temporary/XAI_and_iML_Quotes.tex <==

\cite{confalonieri2021historical} "Explainability is also required by designers and developers to enhance system
robustness and to enable diagnostics to prevent bias, unfairness, and discrimination, as well as to increase trust by all users in why and how decisions are made."
"The goal of extracting explanations via an interpretable global model is to automatically generate general representations of the black-box model and its relationship to features of the dataset is has been trained on." 

\cite{marcinkevivcs2023interpretable} "Interpretable models, sometimes also referred to as “white-” or “gray-boxes,” are usually constrained and structured to reflect physical constraints, monotonicity, additivity, causality, sparsity, or other desirable properties" "explainable ML focuses on introspection for existing black-box models, for instance, by training a simpler surrogate model post hoc. As seen before, explanations can take various forms: textual, visual, symbolic, and so forth. Even a data point from the training set or a synthetic data point can serve as an explanation. An explanation can be global, that is, character- izing the whole dataset, or local, that is, explaining individual classification or regression outcomes. It can be model-specific, that is, capable of explaining only a specific class of models, or model-agnostic, that is, applicable to an arbitrary model."

\cite{markus2021role} "The interpretability  of an explanation captures how  understandable an explanation is for humans. The fidelity of an explanation  expresses  how  accurately  an  explanation  describes  model  behavior, i.e. how faithful an explanation is to the task model. The task  model is the model generating predictions. Hence, they argue an explanation should be understandable  to humans  and correctly  describe  model behavior in the entire feature space." 

\cite{zhou2021evaluating} "Among these terms, explainability and interpretability are more often used than others, and they are also often used interchangeably" "Adadi and Berrada [28] stated that interpretable systems are explainable if their operations can be understood by humans, which shows explainability is closely related to the concept of interpretability. However, Gilpin et al. [29] stated that interpretability and fidelity are both necessary components for explainability. They argued that a good explanation should be understandable to humans (interpretability) and accurately describe model behaviour in the entire feature space (fidelity) [23]. Interpretability is important to manage the social interaction of explainability, while fidelity is important to assist in verifying other model desiderata or discover new insights of explainability. Fidelity is also called faithfulness in some studies [23]."

\cite{schoonderwoerd2021human} "Explainability: the ability to deliver explanations. The model that is  used by the system needs to be interpretable to be able to provide an  explanation (Guidotti et al., 2018b)."
"Causability: the ability the enable a user to achieve causal under- standing with effectiveness, efficiency, and satisfaction in a specified  context of use (Holzinger et al., 2019). 
Interpretability: the ability to provide meaning to a human in un- derstandable terms (Guidotti et al., 2018b)."

\cite{speith2022review} "This is a problem that starts
even outside of taxonomies of explainability methods, for instance, with the lack of a clear distinction between terms like “explainability” and “interpretability” in the XAI debate"

\cite{clinciu2019survey}
"Ribera and Lapedriza (2019) consider that we do not have a concrete definition for
explanation in the literature. However, according
to these authors, every definition relates “explanations with “why” questions or causality reasonings”. "
", we define interpretability
as intersecting with explainability as some models may be interpretable without needing explanations"
"We define interpretable machine learning
as the use of machine-learning models for
the extraction of relevant knowledge about domain relationships contained in data...” (Murdoch et al., 2019)."

\cite{nauta2022anecdotal} 
"1Regarding terminology: “interpretability” and “explainability” are closely related and often used interchangeably in the XAI context [29, 32]. We equate them in this survey as well."
"An explanation is a presentation of (aspects of) the reasoning, functioning and/or be- havior of a machine learning model in human-understandable terms."

\cite{lopes2022xai} 
"Interpretability can be described as the ability to explain in understandable terms to a human"
"explainability is an inherently human-centric property"
"explainability is founded on the “perception and reception of the person receiving the explanation""

\cite{kim2023help}
"umerous explainable AI (XAI) methods have been developed to provide transparency into these AI sys- tems and make them more understandable to people"
"XAI methodscan be categorizedalong several axes: frst, whether amethod is post-hoc or interpretable-by-design;"
"Interpretable- by-design models can provide local and/or global explanations, depending on the model type."
"more interpretable-by-design methods are being proposed; these are typically new types of computer vision models with an explicitly-interpretable reasoning process"

\cite{rong2022towards}
"Methods to increase the interpretability and transparency of an AI system are developed in the research area of Explainable AI (XAI)."
"Explainability is an inherently human-centric property, therefore, the research community should and has started to recognize the need for human-centered evaluations when working on XAI"
"interpretability in ML is defined as the ability to explain or present model predictions in understandable terms to a human. The authors argue that interpretability is used to confirm other important desiderata of AI models such as trust, fairness, or usability"
"Explainability is a human-centric property [151] and therefore XAI should be preferably studied by taking humans’ feedback into account."

\cite{Neupane2022-ly}
"Interpretability is the ability to explain or convey meaning in human-comprehensible terms [64]. This translates into the ability of a human to understand the model’s reasoning without the need for additional explana- tions [65]. On the other hand, explainability is associated with the concept of explanation as a means of interface between humans and a decision-maker (model) that is both accurate and comprehensible to humans [65]"

\cite{Prunella2023-ou}
"interpretability can be defined as a means of finding reasonable evidence in rules of automatic feature selection."

\cite{Sharma2022-tr}
"Explainable artificial intelligence (XAI) generates more interpreta- ble and user-understandable explanations."
"Interpretability is the extent to which an  end-user can acknowledge the source of a decision (Kim  et al. 2016)."
"In machine learning and AI, interpretability and explaina- bility are generally used interchangeably in machine learning  systems. Explainability is the extent to which humans can  understand the internal mechanism of a complex machine  learning system. In comparison, interpretability is the extent  to which we can predict what will happen if the model’s  input parameters have been changed."


\cite{Nor2021-lh}
"pretability refers to the ability to provide human-understandable justification for the one’s behavior. Thus, interpretable AI points to the model’s structures which are transparent and readily interpretable. On the other hand, explainability describes an external proxy used to describe the behavior of the model. Hence, explainable AI refers to post-hoc approaches uti- lized for explaining a black-box model. The first definition explicitly distinguishes between black-box and interpretable models.  The second definition takes a broader connotation where explainability is accented as a technical ability to describe any AI model in general and not only black-box identification."
"XAI approaches are classified according to an explanation scope [41]. Intrinsic models are interpretable due to their simplicity such as in linear regression and logic analysis of data (LAD), while post-hoc approaches interpret more complex nonlinear models [32,33]. Examples of post-hoc approaches are local interpretable model-agnostic explanations (LIME) and Shapley additive explanations (SHAP)."

\cite{molnar2020interpretable}
XAI approaches are classified according to an explanation scope 

\cite{Ogrezeanu2022-ik} 
"n general, explanations are about the attribution of the worth
of input features toward the final model predictions, whereas interpretability refers to the deterministic propagation of information from the input to the response function."

\cite{Ali2023-av}
"rigorous evaluation of  interpretability. Their main contribution is a taxonomy for assessing interpretabil- ity. Consequently, the authors focused on just one element of explainability, i.e., interpretability and its related evalu- ation techniques."
"The word explainability, in terms of AI concepts, means functional knowledge of the model, the purpose of which is to attempt to describe the model’s black-box behavior [28]. It is often used interchangeably with the term interpretability in the literature. Explainability expresses what is occurring in the model by providing a human-readable explanation of the model’s decision. How- ever, it is difficult to come up with a precise description of what qualifies as an explanation. T"
"efinition 3.2.1 (Explainability). The process of elucidat- ing or revealing the decision-making mechanisms of models. The user may see how inputs and outputs are mathematically interlinked. It relates to the ability to understand why AI models make their decisions. The capacity to make auto- matic interpretations and describe the inner workings of an AI system in human terms is referred to as explainability. An explainable technique summarizes the reasons for an AI model’s decision. Furthermore, a model’s "Post-hoc Ex- plainability" refers to methods/algorithms that are used to explain AI model’s decisions [21, 26, 27].
Definition 3.2.2 (Interpretability). Understanding the un- derlying workings of the AI model is another issue with black-box models. The intrinsic properties of a DL model are disclosed through interpretability. This has to do with being able to comprehend how AI models make their decisions. AI systems that explain the internals of an AI model in a manner that humans can comprehend are known as model intrinsic techniques [26, 27, 21]."

\cite{rojat2021explainable}
"Explainability: An ”active characteristic of a model, denot- ing any action or procedure taken by a model with the intent of  classifying  or  detailing  its  internal  functions”  [4],  [5]. ”Given an audience, an explainable Artificial Intelligence is one that produces details or reasons to make its functioning clear or easy to understand"
"Interpretability :   The   passive   characteristic   of   a   model referring to the level at which a given model makes sense for a human observer [4]. An interpretable system is a system where a user cannot only see, but also study how inputs are mathematically mapped to outputs [6]."

\cite{sokol2021explainability}
"In this setting we observe shades of black-boxiness: an interpretability spectrum determined by the extent of understanding exhibited by explainees, which, among others, is conditioned upon their mental capacity and background knowledge."
"alternatively,  interpretability is designated for models and explainability for their outputs (more precisely, reasons behind predictions)"
"The core concept around which we build our nomenclature is explainability; we define it as insights that lead to understanding (the role of an explanation) – a popular and widely accepted rationale in the social sciences"
"interpretability and more re properties of an AI or ML system that enable it to directly (ante-hoc) or indirectly (post-hoc) convey information of varied complexity, the understanding of which depends upon the cognitive capabilities and (domain) expertise of the explainee."

\cite{Vollert2021-tw}
"Every  interpretable  model  [33]  is  also  explainable,  per default  through  introspection  or  through  additional  efforts taken  to  produce  an  explanation"
"As  interpretability  distinguishes  between  models  that  are  in- terpretable  per  introspection  and  models  that  need  additional explanations,  the  terms intrinsic  interpretability and post- hoc  explanations will be used from now on"
"In  this  paper,  we  consider  a  model  as  interpretable  by introspection  if  it  satisfies  the  definition  of  transparency  at the  decomposability  level."

\cite{Ahmed2022-ls}
"deci-
sions, and results must be comprehensible or understandable; in other words, “Explainable.”"


==> SECTIONS/temporary/excluded_papers.tex <==
\cite{Jayawardena2016-ve}
not xai says explainable

\cite{Brinkrolf2018-jt}
mentions pdm but not pdm

\cite{Chen2023-cy}
not a case study



\cite{huf2022cognitive}
not xai or iml

\cite{beretta2021improved}
not xai or iml

\cite{Dang2019-lr}
not predictive maintenance

\cite{Laib_dit_Leksir2018-bi}
isnt xai. It provides the output of 3 algorithms OTSU, Fuzzy CMeans, and SVM. The outputs are fault detection of images which do not have any explanation of how or why the network chose the area. 

\cite{Gribbestad2021health}
say explainability is a focus of the work yet provide no explainability method

\cite{vaccari2022explainable}
reliable ai 

\cite{voronov2021forest}
no interpretation

\cite{konovalenko2022generating}
no interpretation


==> SECTIONS/temporary/explainableAD.tex <==
XAI
\cite{janakiraman2018explaining}precursor
\cite{berno2021machine}diffi
\cite{brunello2023monitors}bSTL
\cite{anello2022anomaly}acme
\cite{marcato2021machine}feature importance
\cite{roelofs2021autoencoder}arcana
\cite{brito2022explainable}shap localdiffi
\cite{glock2021explaining}surrogate
\cite{fan2022incorporating}statistics
\cite{trilla2023unsupervised}causal inference
\cite{kim2021explainable}shap
\cite{lorenti2022cuad}diffi
\cite{ugli2022uzadl}visualization
\cite{lourencco2022using}shap
\cite{mey2022explainable}lrp, gradcam, lime
\cite{Oh2020explainable}cam
\cite{choi2022explainable}shap
\cite{serradilla2021adaptable}Integrated Gradients, SHAP, SmoothGrad
\cite{sanakkayala2022explainable}lime
\cite{hermansa2021sensor}shap
\cite{jakubowski2021anomaly}shap
\cite{jakubowski2021explainable}shap, surrogate
\cite{brunello2020learning}temporal logic, SAX
\cite{jang2019anomaly}LIME
\cite{felsberger2020explainable}LRP
\cite{torcianti2021explainable}LIME
\cite{jakubowski2022roll}counterfactuals, physical constraints
\cite{bellini2021deep}shap
\cite{manco2017fault} feature importance
\cite{ribeiro2022online}rules (AMRules)
\cite{Zhang2021-ee} surrogate
\cite{Ghasemkhani2023-rd} Chi-Squared (feature importance)
\cite{Allah_Bukhsh2019-bk} feature importance
\cite{Li2021-ri} LIME, SHAP
\cite{Hajgato2022-ia} integrated gradients
\cite{Schmetz2021-pf} feature importance

iML
\cite{wang2021ifp}attention
\cite{panda2023ml}decision tree
\cite{yao2023integrated}statistical process
\cite{liu2023causal}graph networks
\cite{xia2022fault}attention
\cite{langone2020interpretable}logistic regression
\cite{michalowska2021anomaly}one class svm
\cite{cao2020using}knowledge based system, SWRL rules,
\cite{xu2021deep}attention
\cite{kothamasu2007adaptive}fuzzy
\cite{salido2004comparison}knowledge based network
\cite{upasane2021big}fuzzy 
\cite{xu2022physics}physical constraints
\cite{lughofer2022transfer} fuzzy
\cite{scott2023computational} MTS
\cite{konovalenko2022generating}k-NN
\cite{Beretta2021-gk} isolation forest for anomaly, gradient boosting for normality
\cite{Upasane2023-al}fuzzy,
\cite{Dhaou2021-qx}Case-crossover APriori (CAP)
\cite{wang2020online}statistical modeling


Both
\cite{li2014improving} rule generation
\cite{steenwinckel2021flags} semantic encoding, knowledge graphs
\cite{matzka2020explainable}feature importance 

==> SECTIONS/temporary/explainableFD.tex <==
XAI
\cite{lourencco2022using} shap
\cite{brito2022explainable}shap, local-DIFFI
\cite{Oh2020explainable}cam
\cite{ERRANDONEA2023103781}surrogate
\cite{BRITO2023120860}grad-cam
\cite{steurtewagen2021adding}shap
\cite{keleko2023health}deepshap
\cite{mylonas2022local} LionForests
\cite{Remil2021-kr}feature importance
\cite{Han2022-yk}LRP

iML
\cite{xia2022fault}attention
\cite{verkuil2022automated}fault tree
\cite{li2022waveletkernelnet}interpretable filters
\cite{li2023wavcapsnet}interpretable filters
\cite{pu2023restricted}sparse networks
\cite{xin2022fault}fourier transforms
\cite{ben2022end}interpretable filtesr
\cite{hafeez2022dtcencoder}attention
\cite{ming2019interpretable}prototype
\cite{yang2022noise}gam
\cite{kothamasu2007adaptive}fuzzy
\cite{chen2020temporal} STL
\cite{Mahmoodian2022-zk}digital twin
\cite{Xia2023-bg} knowledge graphs

==> SECTIONS/temporary/explainableProg.tex <==
XAI
\cite{wu2018k} rule-based
\cite{gashi2023impact} shap
\cite{sanakkayala2022explainable}lime
\cite{sayed2022explainable}shap
\cite{serradilla2020interpreting}ELI5, LIME
\cite{khan2022explainable} LIME, SHAP
\cite{Solis-Martin2023-po} SHAP, LIME, Grad-CAM, LRP, Image-Specific Class Saliency Maps
\cite{Alfeo2022-or}feature importance, LIME
\cite{Wang2023-px}LRP
\cite{Simmons2021-hj} feature impotrance
\cite{Protopapadakis2022-ye}LIME
\cite{Jakubowski2022-hh} SHAP, LIME 
\cite{Ferraro2023-jv} LIME, SHAP
\cite{Bakdi2022-gw} feature importance
\cite{Kononov2023-ys} SHAP
\cite{voronov2021forest} feature importance\\

iML
\cite{yang2022noise} GAM
\cite{costa2022variational} latent representations
\cite{Ding2021-ez}  symbolic life models
\cite{Amram2021-gt} decsion tree
\cite{Tod2023-cf} physical model
\cite{Abbas2022-mm} HMM
\cite{Jing2022-yq} attention
\cite{Waghen2022-na} fault tree
\cite{csalodi2021mixture} gaussian mixture model
\cite{Jakubowski2022-hh} Explainable Boosting Machine
\cite{Castle2020-pc} Bayesian and frequentist model

==> SECTIONS/temporary/survey_summaries.tex <==
\cite{janakiraman2018explaining}
\begin{itemize}
    \item The authors model safety incidents with a new architecture called Deep Temporal Multiple-Instance Learning (DT-MIL) which is a combination of MIL and Deep Recurrent Networks (DRNN). The MIL has the ability to learn using weakly supervised data while the DRNN is used to model the temporal dependencies. To explain the safety events, the authors utilize precursor mining to determine where in a time series vector a safety incident occurs using probability. With all of these different techniques, their model learns high-level safety incidents and uses DT-MIL to correlate the high-level safety events to low-level instances.
    \item XAI
    \item Deep Temporal Multiple-Instance Learning (DT-MIL), GRU with DNN
    \item Flight operational quality assurance data
    \item Precursor analysis/mining 
    \item Area under the ROC curve (AUC), 0.9904 train/ 0.9837 test
    \item None
\end{itemize}

\cite{wang2021ifp}
\begin{itemize}
    \item The authors propose a two-stage interpretable fault prediction method based on anomaly detection and anomaly accumulation. The anomaly detection module is made using a CT-GAN to train a discriminator on limited data, i.e. faults. The anomaly scores that are output by the anomaly detection module are fed into the anomaly accumulation module which is based on an Attention-LSTM. The LSTM is used to model the temporal dependencies of the anomaly scores while the Attention mechanism is used to give importance to different anomalies at different time steps. Their model outperforms models such as SVM and LSTM on prediciton and DTW on classification.
    \item iml
    \item 2 stage model: CT-GAN for anomaly detection and Attention-LSTM for fault prediction
    \item IOV (vehicles) and AIC (air conditioners)
    \item feature importance can be seen using the correlation matrices in CT-GAN
    \item precision, recall, f1-score
    \item none
\end{itemize}

\cite{berno2021machine}
\begin{itemize}
    \item The authors model gives enhanced monitoring capabilities to the enertainment industry in the form of anomaly detection for automated rides for entertainment parks. Their data is split into two types: multivariate smart monitoring features and univariate specified signals. They utilize isloation forest to model the multivariate time series with Depth-based Feature Importance for the Isolation Forrest (DIFFI) explaining the output. They model the univariate time series with a Growing When Required (GWR) neural gas network.
    \item XAI
    \item isolation forest for multivariate, growing hen required neural gas network for univariate
    \item park rides
    \item Depth-based Feature Importance for the Isolation Forrest (DIFFI) 
    \item none
    \item none
\end{itemize}
\cite{brunello2023monitors}
\begin{itemize}
    \item The authors use an evolutionary approach to fault detection. They utilize Distributed Evolutionary Algorithms in Python (DEAP) to alter syntax trees that contain bounded signal temporal logic (bSTL) statements, which are an extension to propositional logic that expresses temporal properties. They use these statements both as a way of fault detection and as a way of simply explaining using the features. They test their method on 3 datasets: Blackblaze Hard Drive, Tennessee Eastman Process, and CMAPSS. While their method was not the best performing, they had very good performance in precision, recall, FAR, and F1-score all around in the 3 datasets.
    \item XAI
    \item Evolutionary algorithm with Trees
    \item Blackblaze Hard Drive, Tennessee Eastman Process, CMAPSS
    \item bounded signal temporal logic (bSTL)
    \item precision, recall, FAR, F1
    \item none
\end{itemize}

\cite{anello2022anomaly}
\begin{itemize}
    \item The authors apply a newer explainability method, accelerated-agnostic explanations (AcME), to the problem of anomaly detection as to compare it to SHAP. They utilize isolation forest to detect anomalies as it is commonly used for detecting outliers or anomalies. They use the anomaly score as a label for the time series to represent the problem as a regression task. This is done so AcME can be used as it has only been applied to regression tasks. They apply both SHAP and AcME to anomaly detection for a roller coaster dataset and a compacting machine dataset. Their main finding was the drastic speed up by using AcME with all of the data while SHAP would be slow even with access to 30\% of the data.
    \item XAI
    \item isolation forest 
    \item roller coaster and compacting machine
    \item accelerated-agnostic explanations (AcME) 
    \item none
    \item none
\end{itemize}

\cite{marcato2021machine}
\begin{itemize}
    \item The authors main contribution is applying and evaluating multiple anomaly detection models for particle accelerators. They apply k-nearest neighbors, local outlier factor (LOF), clustering based local outlier factor (CB-LOF), feature bagging with LOF base, lightweight online detector of anomalies (LODA), and isolation forest. Not only do they apply these models to a particle accelerator, they use permutation feature importance to guide model development. The feature importance allows them to find the optimal sliding window with the most useful features. This allowed them to show CB-LOF to be the best model in terms of TP, FP, FN, precision, recall, and F-score.
    \item XAI maybe
    \item k-nearest neighbors, local outlier factor (LOF), clustering based local outlier factor (CB-LOF), feature bagging with LOF base, lightweight online detector of anomalies (LODA), and isolation forest
    \item one month long shift of the ALPI accelerator
    \item permutation feature impotance maybe
    \item TP, FP, FN, precision, recall, f-score
    \item none
\end{itemize}

\cite{scott2023computational} 
\begin{itemize}
    \item The authors introduce using the Mahalanobis-Taguchi system for fault detection. MTS utilizes Mahalanobis distance, orthogonal arrays, and signal-to-noise ratios for multivariate diagnosis and prediction. The Mahalanobis space represents the stable operations and would output how different a observation is from stable. The orthogonal arrays and signal-to-noise ratio is used to diagnose or identify variables responsible for the fault. They show MTS aplied to a predictive maintenance example from the University of California Irvine
    \item iml
    \item None
    \item UCI  Machine  Learning   Repository,
    \item none
    \item none
    \item none
\end{itemize}

\cite{panda2023ml}
\begin{itemize}
    \item The authors aimed at tackling the problem of commercial vehicle predictive maintenance by designing an interpretable ML framework. To simplify their problem, they solely looked at the air compressor system. With just looking at the air compressor system, they ran an broad experiment that looked at different configurations of model and data. They found the C5.0 with boosting model performed the best, and they found including Diagnostic Trouble Codes with the sensor data raised the performance metrics generally.
    \item iml
    \item C5.0, C5.0 with boosting, Classification adn Regression Tree (CART) (decision trees)
    \item electronic air compressor systems in vehicles
    \item inherent explainability of decision trees
    \item accuracy, specificity, recall, precision, AUC, Gini
    \item none
\end{itemize}

\cite{roelofs2021autoencoder}
\begin{itemize}
    \item The authors build a novel method for root cause analysis in anomaly detection by building on top of the basic autoencoder. The difference in reconstruction (reconstruction error) can identify when an anomaly occurs, but it cannot define the cause of the anomaly. The authors propose Autoencoder-based anomlay root cause analysis (ARCANA) as an optimization algorithm to overcome this limitation. The model's main assumption is that even if only one or two input features show an error, the error is propagated through the network. ARCANA searches deviating input features while trying to find onlya  few explanatory features by minimizing their loss function. ARCANA provides a list of features and their importance to the output which explains the reconstruction error, i.e. the anomaly.
    \item xai
    \item autoencoder
    \item Open Wind Farm data set (wind turbines)
    \item ARCANA
    \item none
    \item none
\end{itemize}

\cite{yao2023integrated}
\begin{itemize}
    \item The authors propose a framework with interpretable and automatic approaches that consists of solely statistical processing. Their method proposes kurtosis-energy metric to define key sub-bands, a new health index of these sub-bands, a joint statistical alarm and fault identification strategy and a health phases segmentation strategy for health phases assessment and degradation pattern analysis. This method involves analyzing the data on the time-frequency domain and suppressing the disturbing components such as noise. This analysis is able to help form the sub-bands which are then used for monitoring the current state. If it fails statistical test, then an anomaly is detected. They test their method on the PHM 2012 rolling bearing dataset, and they report very low false positives from their method. 
    \item iML
    \item statistical modeling
    \item Rolling bearing
    \item unclear but most likely its the visualization of their new HI method
    \item false alarm count
    \item none
\end{itemize}

\cite{brito2022explainable}
\begin{itemize}
    \item The authors perform a large experiment that applies many unsupervised learning algorithms for fault detection and fault diagnosis. First, they proposed a framework that consisted of fault detection, explainability, root cause analysis and unsupervised fault classification. They showed that Local-DIFFI and SHAP seem to be mostly in agreement about the explanation for the model's output, but they do not move further in asking which is better. 
    \item XAI
    \item KNN, minimum covariance determinant, local outlier factor, one-class support vector machines, feature bagging, isolation forest, histogram-based outlier score, ensemble
    \item bearings, gearbox, mechanical fault
    \item SHAP, Local-DIFFI
    \item AUC, F1-score, time
    \item There was not an evaluation of "good" explanations but the outputs of both SHAP and DIFFI were compared and shown to be similar
\end{itemize}

\cite{glock2021explaining}
\begin{itemize}
    \item The authors propose a unique method of explaining a black-box model by using explainable surrogate models. They train a random forest model and an ARIMA model on the same data. From this they can gather the residual error from the RF model. Then a separate ARIMA model is trained to predict the residual error from the RF model. Through a comparison of the two ARIMA models, one can observe what the RF model is able to learn and not learn from the data. 
    \item XAI
    \item Random forest
    \item machine failure
    \item surrogate models (ARIMA)
    \item none
    \item none
\end{itemize}

\cite{liu2023causal}
\begin{itemize}
    \item The authors designed a framework for fault detection based around the Graph Convolutional Network and Graph Attention Networks. They propose the Causal-GAT. Causal-GAT is comprised of two parts: causal graph construction and DC-Attention for extracting features and detection. The causal graph construction uses causal discovery methods and/or prior expertise to encode monitoring variables into a directed acyclic graph. The Disentangled Causal Attention (DC-Attention) aggregates the causal variables for generating representations of the effect variables. The DC-Attention outputs the system status (faulty or not faulty). They then utilize a custom loss function that calculates the distance between the current support of representations and its theoretically disentangled support. 
    \item iml
    \item Causal Graph Attention Networks
    \item high-speed train braking systems
    \item GNN Explainer
    \item F1, G-mean
    \item none
\end{itemize}

\cite{xia2022fault}
\begin{itemize}
    \item The authors propose a framework based on deep learning and hierarchical attention to make the process of fault diagnosis interpretable. Their method breaks down AUV's into different layers of information in a hierarchical way, i.e. vehicle into subsystem into components to sensors. They utilized BiLSTM encoders and attention to obtain important features and detect faults, and they used random masking and feature orthogonalization to make the weights of the network interpretable. This architecture was applied to AUVs with plans of expanded their use cases.
    \item iML
    \item  hierarchical attention based multi-source data fusion method for AUV fault diagnosis (HAMFD) (bilstm - attention)
    \item Qianlong-2 AUV
    \item attention
    \item fault detection rate, false alarm rate, precision, accuracy, F1
    \item none
\end{itemize}


\cite{fan2022incorporating}
\begin{itemize}
    \item The authors  join the trend of developing ML methods that take advantage of physics knowledge for added interpretability. Their case study is fault detection of leak-related faults in vehicle air systems. They fit 3 physics equations to their data that would model the air leakage. They then use that data in the training data of their kNN and MLP models. Results show that the physics-assisted models outperform the non-assisted models. 
    \item XAI
    \item physics assisted knn and mlp
    \item vehicle air system
    \item ANOVA F-score
    \item AUC
    \item none
\end{itemize}

\cite{mylonas2022local}
\begin{itemize}
    \item The authors aim at alleviating the non-explainable nature of random forest by applying a recent method called LionForests. They expand LionForests into the realm of multi-label classification. They expand it by three different strategies: single label, predicted labelset, and label subsets. Single label aims at explaining based every individual prediction (local); predicted labelset aims at explaining all predictions (global); and label subsets aim at explaining based on frequently appearing subsets of predictions. They apply their method to many datasets including a synthetic machine failure dataset. They apply metrics of explainability and performance while comparing their algorithm to other explanation algorithms namely global and local surrogates and Anchors.
    \item iml
    \item Random Forests
    \item AI4I (synthetic dataset of machine failures)
    \item Lion Forest
    \item precision and time response
    \item rule length, coverage of data, comparison to other explainable methods
\end{itemize}

\cite{trilla2023unsupervised}
\begin{itemize}
    \item The authors design an anomaly detection framework based around a denoising variational autoencoder (VAE) and a MLP. They extract intrasubsystem and intersubsystem patterns via making the time series data into voxels. The VAE generalizes the embeddings. Finally the MLP  is used to create a smooth diagnosis probabilistic function. They apply their method on a locomation dataset and utilize causal inference via the Peter-Clark algorithm to answer the question "Did the VAE learn cause-effect relationships?" They found that the VAE could at best be described as modeling a correlation relationship, but mainly due to data availability. 
    \item XAI
    \item VAE
    \item locomation data
    \item Causal inference via Peter-Clark algorithm
    \item precision and recall 
    \item none but they at least question the validity of their explanations
\end{itemize}

\cite{kim2021explainable}
\begin{itemize}
    \item The authors propose performing anomaly detection on maritime engines. With explainability in mind, they propose using isolation forest for anomaly detection and SHAP to explain the output of the isolation forest. While this was a large portion of their work, they also perform hierarchical clusing analysis with the SHAP values as to group common anomalies. 
    \item XAI
    \item isolation forest
    \item maritime engine 
    \item SHAP
    \item none
    \item none
\end{itemize}

\cite{verkuil2022automated}
\begin{itemize}
    \item The authors notice that fault trees are made via human intervention. With a large amount of data, they wanted to try to automatically make fault trees via learning algorithms. They combine C4.5 and LIFT to create fault trees for domestic heaters. C4.5 is used to learn the failure thresholds of the sensor data. LIFT takes that information and creates fault trees in an iterative process. While they do not provide a performance metric, they note that their method cannot be optimal for the reasons of oversimplifying the problem and using a greedy heuristic. They provide many explanations from their model, and domain experts weigh in on the explanations in a positive manner.
    \item iML
    \item fault trees
    \item heaters
    \item tree
    \item none
    \item advice from domain experts
\end{itemize}

\cite{lorenti2022cuad}
\begin{itemize}
    \item The authors design an unsupervised and interpretable anomaly detection pipeline known as Continuous Unsupervised Anomaly Detection on Machining Operations (CUAD-MO). CUAD-MO consists of 4 parts: data segmentation and feature extraction, unsupervised feature selection via Forward Selection Component Analysis (FSCA), anomaly detection via Isolation Forest, and post-hoc explainability via DIFFI. They apply their method to 2 years of computer numerical control data, and they show 67\% precision. 
    \item XAI
    \item Isolation Forest
    \item Computer Numerical Control data
    \item DIFFI
    \item Confusion matrix
    \item none
\end{itemize}

\cite{ugli2022uzadl}
\begin{itemize}
    \item The authors aim to add interpretability to automated visual inspection for anomaly deteciton. They propose UzADL, a 3 stage system that consists of pseudo-labeling of data, training via a deep convolutional network, and illustrating of locations of defects. For pseudo-labling, the authors utilize Laplacian matrices to break the unlabeled data into two clusters, verified via Silhouette coefficient. They use transfer learning by using ResNet-18 as opposed to training a DCNN from scratch. Finally, they locate defective regions of anomalies via calculating significance of the pre-final layer of the DCNN for anomalous instances. They use 3 datasets to test their method and compare it to 5 other methods. Their main findins show that their method performs the best, but not as good as they want it to be performing.
    \item XAI
    \item ResNet-18
    \item NanoTWICE, MVTec AD, and DWorld
    \item visualization
    \item  accuracy, false positive, true positive or recall, precision, f1
    \item they gave opinions of the quality of the heatmaps, but not the accuracy
\end{itemize}

\cite{lourencco2022using}
\begin{itemize}
    \item The authors perform fault detection and fault diagnosis for plastic extruders. For fault detection, they utilized isolation forests. For fault diagnosis, they used SHAP to explain their isolation forest. They used this explanation as the fault identification/root cause. 
    \item XAI
    \item isolation forest
    \item plastic extruders
    \item SHAP
    \item none
    \item none
\end{itemize}

\cite{mey2022explainable}
\begin{itemize}
    \item This work focuses on the plausibility of XAI methods for explaining a CNN model. They test the plausibility via a synthetic dataset, and they then apply it to a real problem. They investigated GradCAM, LRP, and LIME to generate visual explanations of their model. In these explanations, they found that GradCAM highlighted everything as it was supposed to, LRP highlighted factors that were not distinguishable to any class, and LIME highlighted some of the features that were unimportant. They also found that LRP had a high false-positive rate with its explanations when compared to the others, i.e., pixels were incorrectly highlighted as relevant. When they moved their methods to a real-world problem, the performance of the XAI algorithms showed to be slightly worse in some cases. 
    \item XAI
    \item CNN
    \item synthetic and rotating machine
    \item LRP, GradCAM, LIME
    \item Accuracy
    \item They used a synthetic dataset that had inherent interpretability. They used this as a benchmark for comparing the different xai methods. While this does not directly translate to the real data, it is an interesting way of comparing the validity of explainable methods.
\end{itemize}

\cite{Oh2020explainable}
\begin{itemize}
    \item This paper proposes a fault detection and diagnosis framework that consists of a 1D-cnn for fault detection, class activation maps for fault diagnosis (explainable method) and VAE for implementing user feedback. The CNN utilizes a GAP layer as the output layer due to its ability to maintain the temporal information. This also allows them to use CAM as an explainable method as opposed to GradCAM. The VAE is utilized with the principle of Garbage-In, Garbage-Out logic to minimize the amount of false positives and negatives that would be presented to the users. To verify their method, they apply it to the Ford Motor dataset which is a vehicle engine dataset that contains an amount of noisy data. They show that their model is accurate even in noisy data, and they show that the VAE increases their accuracy. They also show via CAM that the anomalous data is linearly separable, which is found in the VAE. 
    \item XAI
    \item 1D-CNN
    \item Ford Motor
    \item CAM
    \item accuracy
    \item using a VAE they can lower the amount of false explanations
\end{itemize}




\cite{li2022waveletkernelnet}
\begin{itemize}
    \item The authors aim to improve upon CNN based methods for PHM by addressing the black box problem. They propose the Continuous Wavelet Convolution layer which is designed to make the first layer of a CNN interpretable. It does this by using a library of filters that have physical meaning which are convolved on the input signal. These convolutions can be traversed along the series and project it into a two-dimensional time and scale dimension. Its performance is compared with a base CNN with different wavelets, and they showed 1) their model outperformed the CNN and 2) their wavelet convolution layer learned with a well definied waveform while the CNN looks noisey and uninterpretable. 
    \item iML
    \item CNN with continuous wavelet convolution layer, aka waveletKernelNet
    \item bearing, gears
    \item utilizing waveforms to explain what the network is learning
    \item accuracy
    \item none
\end{itemize}

\cite{li2023wavcapsnet}
\begin{itemize}
    \item The authors perform fault diagnosis with the specific aim at compound faults. They design an interpretable framework called wavelet capsule network (WavCapsNet) which utilizes backward tracking. This network has 1) interpretable meaning from the wavelet kernel convolutional layer, 2) capsule layers that allow decoupling of the compound fault, and 3) backward tracking which helps interpret output by focusing on the relationships between the features and health conditions. Not only is there framework able to achieve high accuracy on all conditions, including compound faults, but also they show that the backward tracking method can decouple the capsule layers effectively.
    \item iML
    \item WavCapsNet, CNN with wavelet kernel conv layers and capsule layers for decoupling
    \item vehicle transmission
    \item feature extraction using inherently explainable layers and backtracking to locate the discriminative features that determine the fault diagnosis
    \item accuracy
    \item show that backward tracking is able to decouple via masking discriminative features and analyzing performance
\end{itemize}

\cite{pu2023restricted}
\begin{itemize}
    \item This works explores a new frequency domain space they call the restricted sparse frequency domain space (RSFDS) for rolling bearing faults. The RSFDS breaks down the features into a space that is made of real and imaginary points. This space is able to visualize boundaries that have physical meanings to the faults. They use a simple two-layer neural network to these points, and they achieve high performance equal to that of a CNN-LSTM with less memory and CPU usage. 
    \item iML
    \item Restricted sparse networks
    \item rolling bearings
    \item inherent interpretability of network
    \item accuracy
    \item none
\end{itemize}

\cite{xin2022fault}
\begin{itemize}
    \item The authors aim to address bearing fault diagnosis by utilizing a novel model logarithmic-short-time Fourier transform modified self-calibrated residual network (log-STFT-MSCResNet). The STFT extracts time-frequency features from raw signals to retain physical meaning of fault signatures. The MSCResNet is used to enlarge the receptive field without introducing more parameters. With the combination of the two, they aim to have high accuracy even under unknown working conditions. They compare their model to popular models such as LSTM and ResNet18. log-STFT-MSCResNet performs among the best, has a small amount of features, and trains in a shorter time than some of the larger models tested. This model also performs very well on faults that are not in the training data.
    \item iML
    \item log-STFT-MSCResNet (logarithmic short-time Fourier transform modified self-calibrated residual network)
    \item bearings
    \item inhrent interpretability
    \item accuracy and confusion matrix
    \item none
\end{itemize}

\cite{ERRANDONEA2023103781}
\begin{itemize}
    \item The authors take the theoretical approach of applying XAI on edge computing to the application domain for fault diagnosis of train wheelsets. They use H2O.ai's AutoML to perform their fault diagnosis. They utilize all possible models while balancing accuracy and hardware requirements, and they enfore the hardware requirement via Docker and Java. They also balance interpretability of the selected models by weighing feature sensitivity and the effect of the features on the target variable via individual conditional expectation and partial dependency. This is used to create a post-hoc interpretable surrogate model. 
    \item XAI
    \item automated, ends up being an ensemble
    \item train wheelset
    \item automated, ends up being a surrogate model
    \item ram usage, cpu usage, prediction execution time, accuracy
    \item explainability analysis via feature sensitivity, feature effects, and developing the interpretable model
\end{itemize}

\cite{BRITO2023120860}
\begin{itemize}
    \item They utilize transfer learning to overcome weaknesses of supervised learning such as low faults and labeled data. They generate signals from the different faults in the dataset, and combine them with the original signals of the machine. They train their model on this data, and they test the model on the real data. Their model was able to perform well in the new domains, and they are explained via Grad-CAM to increase user trust. 
    \item XAI
    \item 1D CNN
    \item bearing, gearbox, mechanical faults
    \item Grad-CAM
    \item accuracy
    \item none
\end{itemize}

\cite{ben2022end}
\begin{itemize}
    \item The authors propose a new DL architecture that trains directly on the raw vibration signals to diagnose bearing faults. Their architecture builds off of CNNs by replacing the first convolutional layer with interpretable digital filters. They can reduce the number of trainable parameters and extract meaningful representations by having the predefined functions serve as the convolution. When comparing the performance to a CNN, the SincNet has a higher precision and reaches convergence faster.
    \item iML
    \item Deep-SincNet (an interpretable CNN)
    \item bearings
    \item interpretable first layer
    \item AUC and accuracy
    \item none
\end{itemize}

\cite{wang2020online}
\begin{itemize}
    \item iml
    \item detection
\end{itemize}



\cite{wu2018k}
\begin{itemize}
    \item The authors propose the K-PdM (KPI-oriented PDM) framework, a cluster-based HMM based on key performance indicators (KPIs). Each KPI is one dimension of fine-grained deterioration, and combination of KPIs reflects the overall HI and RULs of machine. T K-PdM is two-phases: fine-grained deteriorating mode and overall deterioration estimation along with RUL prediction. The fine-grained deteriorating mode consists of clustering to convert KPI time series into symbolic sequences, HMM initialization according to the symbolic sequence and finally obtaining optimal state sequence via extended Viterbi. The deterioration estimation and RUL prediction phase consists of estimating current deteriorating state based on the given KPI sequence, a linear polynomial regression model for predicting RUL and root-cause analysis via a semantic rule-based reasoner. They applied their method to CMAPSS dataset, and they showed a high, not highest, accuracy. 
    \item XAI
    \item cHMM
    \item NASA Turbofan
    \item semantic rule-based reasoner
    \item AE, RMSE
    \item None
\end{itemize}


\cite{hafeez2022dtcencoder}
\begin{itemize}
    \item The authors perform DTC prediction which can be analogous to fault diagnosis. Instead of using an LSTM or some other explicit black-box method, they design an architecture called DTCEncoder. DTCEncoder learns low compact representations of multivariate sequences with attention. Their model firstly trains an LSTM architecture with attribute embeddings to learn a hidden state. They apply the attention  mechanism to gain a context-vector of the hidden states. The context-vector is passed through some dense layers to obtain an encoding of the sequence. It then outputs into more dense layers to determine the probability of the different attributes for DTC prediction. For interpretability, they take the output of the DTCEncoder and apply t-SNE to reduce the dimensions and visualize them. 
    \item iML
    \item Diagnostic Trouble Codes Encoder (DTCEncoder)
    \item Vehicles
    \item attention
    \item accuracy
    \item none
\end{itemize}

\cite{li2014improving}
\begin{itemize}
    \item The authors perform failure prediction with a combination of two methods. Fristly, they perform alarm prediction,a specific failure prediction, using an SVM based model. To make the output human-readable, they perform an exhaustive search among the feature space and visualize the first two principle components. With the visualization they are able to make some basic rules that predict the alarm. For failure prediction, specific failures besides general alarm, they use a decision tree, and they generate the rules form the decision-trees for interpretability. 
    \item both
    \item Decision tree and SVM
    \item train
    \item inherent interpretability 
    \item true positive and false positive
    \item none
\end{itemize}

\cite{choi2022explainable}
\begin{itemize}
    \item The authors propose a method for explainable unsupervised anomaly detection to predict system shut downs for chemical processes. Their method consists of what they call a period-independent framework and a period-integrated framework. The period-independent framework searches for the best anomaly detection model and applies the explainable method. In this framework, they test window kernel density estimation, local outlier factor, one-class SVM, isolation forest, autoencoder, variational autoencoder, LSTM autoencoder, multi-scale convolutional recurrent encoder-decoder, and BeatGAN. In the period-integrated framework, they apply real-time information to the model chosen from the previous framework. They find that the isolation forest provided the best results in the period-independent framework based on the amount of unplanned shutdowns detected, and thus, apply it to the period-integrated framework. They utilize SHAP to serve as a root cause analysis or fault diagnosis method based on the detected anomaly. 
    \item XAI
    \item window kernel density estimation, local outlier factor, one-class SVM, isolation forest, autoencoder, variational autoencoder, LSTM autoencoder, multi-scale convolutional recurrent encoder-decoder, and BeatGAN
    \item chemical process
    \item SHAP
    \item false alarm rate, accuracy
    \item Evaluation of explanation if given
\end{itemize}

\cite{langone2020interpretable}
\begin{itemize}
    \item The authors propose a model for interpretable anomaly prediction based on a logistic regression model with elastic net regularization. As opposed to anomaly detection, they perform anomaly prediction. Their method is made of 3 steps: data preparation, learning and refinement of the prediction model. In the data preparation portion, they bucket the data with statistics included in the data; they window the data; finally, they flag the windows as anomalous or not. The learning phase consists of learning the relevant features from the windowed data. This consists of considering the feature distributions across failures and non-failures and measuring the distance according to the Kolmogorov-Smirnov metric. The refinement of prediction model phase consists of the training and utilization of the logistic regression model. Coupled with elastic net regularization, this model selects a smaller subset of the original data and captures the variable correlations. They apply their method to a plunger pump in a chemical plant, and they show relative good and consistent scores. 
    \item iML
    \item logistic regression with elastic net regularization model
    \item high pressure plunger pump in chemical plant
    \item feature importance 
    \item cohen's kappa, AUC, PRAUC, precision and recall
    \item none
\end{itemize}

\cite{ribeiro2022online}
\begin{itemize}
    \item Summary
    \item XAI
    \item Model
    \item Dataset
    \item Explainable Method
    \item Evaluation of model
    \item Evaluation of explanation if given
\end{itemize}

\cite{serradilla2021adaptable}
\begin{itemize}
    \item The authors performed semi-supervised deep learning for anomaly detection. Their main algorithm was the 2D-CNN-AE that was trained soley with correct working machine data. To add interpretability to their model, they utilized gradient explainer from SHAP library which includes Integradted Gradients, SHAP, and SmoothGrad. They also showed that their method encoded the data meaningfully by using t-SNE and SOM for projecting the latent space into a 2D space. They also showed that their model is adaptable to data variations via transfer learning with only a small amount of added training. 
    \item XAI
    \item PCA, extreme learning machine, OCSVM, 2D-CNN-AE, null space
    \item press machine
    \item gradient explainer combines Integrated Gradients, SHAP, and SmoothGrad into a single expected value equation.
    \item f1
    \item none
\end{itemize}

\cite{gashi2023impact}
\begin{itemize}
    \item The authors perform predictive maintenance on a multi-component system where they aim to model interdependencies and test their importance. Prior to training their Random Forest model, they use visual exploration to view where there are interdependencies. They use two methods to justify the use of interdependencies: statistics and XAI. The use chi-squared testing to show that the performance of a model with independencies as variables performs better than one without (p < 0.001). When applying SHAP to the random forest, they can show that the interdependency variables are usually there among the top explainer features. 
    \item XAI
    \item Random Forest
    \item semi-conductor
    \item SHAP
    \item precision, recall, f1, support
    \item Evaluation of explanation if given
\end{itemize}

\cite{sanakkayala2022explainable}
\begin{itemize}
    \item The authors create a framework that performs both RUL prediction and fault detection. Their main contribution involves transforming time series data into a spectrogram. This allows them to visualize unusual bands that may indicate faults. They apply unsupervied clustering of the spectrograms in the form of K-Means clustering to partition the data into healthy and unhealthy. They use a large CNN model (VGG16) for fault detection which uses LIME to explain the results. Finally they use a simpler CNN model for RUL prediction. 
    \item XAI
    \item VGG-16 for fault detection, 2 layer CNN for RUL
    \item bearing
    \item LIME
    \item accuracy, recall, f1 for detection, RMSE, MSE, R2 for RUL
    \item none
\end{itemize}

\cite{hermansa2021sensor}
\begin{itemize}
    \item The authors propose a framework that is made of two separate models: a base model and a correction model. The base model is used for anomaly detection. In their use case they test HDBSCAN, LOF, isolation forest, and OCSVM. An XAI method, in this case SHAP, is used to explain the output of the base model. When an anomaly is detected, the correction model, in this case a random forest, is launched. This model limits the number of alarms reported to the operator by confirming the anomaly. The operator has a chance of confirming the alarm. The correction model is refined given the operator's input. They test their method on coal machinery and find that 1) HDBSCAN shows to have the best performance in their case and 2) the correction model betters the performance.
    \item XAI
    \item HDBSCAN, LOF, isolation forest, OCSVM, RF
    \item coal machinery
    \item SHAP
    \item P (percentage of true outliers), N (ratio of normal values marked as outliers vs the number of all non-outlier values) and Score (interaction between the two above)
    \item none
\end{itemize}

\cite{jakubowski2021anomaly}
\begin{itemize}
    \item This is an extension to \cite{jakubowski2021explainable}. The authors aim to use unsupervised learning in the form of a Variational Autoencoder for anomaly detection. The detection in done by via reconstruction error. Then they train a Random Forest Classifier where the inputs are the data and the outputs are the anomaly label given by the VAE. SHAP is then used to explain this surrogate model's outputs. They apply their method to both CMAPPS and Hot Rolling. 
    \item XAI
    \item variational autoencoder and RF
    \item CMAPSS and hot rolling
    \item SHAP
    \item accuracy, precision, recall, F1
    \item none
\end{itemize}

\cite{lughofer2022transfer}
\begin{itemize}
    \item Summary
    \item iML
    \item Model
    \item Dataset
    \item Explainable Method
    \item Evaluation of model
    \item Evaluation of explanation if given
\end{itemize}

\cite{michalowska2021anomaly}
\begin{itemize}
    \item The authors propose a two phase framework for anomaly detection that consists of unsupervised anomaly discovery and semi-supervised construction and tuning of an anomaly detection algorithm. The anomaly discovery phase uses many techniques such as PCA and Kolmogorov-Smirnov test for feature significance. They then used domain knowledge to narrow down the determined most important features to make the feature pool smaller. Their algorithm construction phase consists of utilizing a One-Class SVM to represent normal behavior versus anomalous behavior. After model training, they inspect false positives with the assistance of experts to update their model to handle these instances. 
    \item iML
    \item one class svm
    \item maritime
    \item visualization of features
    \item none
    \item domain experts are used to a) pick potential features and b)the features picked are indicative of anomalies
\end{itemize}

\cite{steenwinckel2021flags}
\begin{itemize}
    \item The authors produce a framework for anomaly detection and root cause analysis. They introduce Fused-AI Interpretable Anomaly Generation System (FLAGS) which combines knowledge-driven and data-driven techniques to gain the benefits of both and negate the detriments. Their framework is made of 3 parts: anomaly detection, fault recognition and root cause analysis  to create semantic and interpretable anomalies and faults, a dashboard to capture user feedback, and an optimization of the anomaly detection and root cause analysis through fused AI and user feedback. The first phase combines both knowledge-driven and data-driven approaches of AD, FR, and RCA to create a semantic database of rules. The second part displays the rules from the semantic database and allows for user feedback. The third part uses the feedback to optimize the data-driven models via feature engineering and correcting the models, verify semantic rules, and add knowledge/rules to the knowledge driven approaches. For the knowledge-driven method, they use knowledge graphs. For the data-driven method, they used Matrix Profile. They showed high accuracy when applied to a train dataset, and they illustrated the adaptability of their method by utilizing input given from the train operators.
    \item both
    \item knowledge graph, matrix profile
    \item trains
    \item semantic encoding and knowledge graphs
    \item Evaluation of model
    \item Evaluation of explanation if given
\end{itemize}

\cite{jakubowski2021explainable}
\begin{itemize}
    \item The authors utilize a quasi-autoencoder for explainable anomaly detection. It uses both stationary data and sequential data in the encoder to create sequential data in the decoder. They tested their method on hot-rolling steel, and they achieved a high $R^2$ score. To add explainability, they used a surrogate model (XGBoost) and TreeExplainer (SHAP) to show the features with highest impact on the classification. 
    \item XAI
    \item quasi autoencoder, combination of LSTM and FC layers in autoencoder
    \item artificial dataset and hot-rolling steel
    \item SHAP of XGBoost
    \item AE got a .88 + r-2 score, but the gradient boosting surrogate model got .98.
    \item none
\end{itemize}

\cite{brunello2020learning}
\begin{itemize}
    \item The authors show that they are able to apply monitoring with machine learning to perform anomaly detection in an online setting. Their method is modular where it can be applied in a semi-supervised and unsupervised manner, depending on if they received or did not receive expert knowledge prior respectively. They system is in a constant state of monitoring. Once a failure is detected, the monitoring system extracts the failure trace, a time segment that is close to the failure event, and a normal trace, the rest of the time window prior to the failure trace. The traces are used to create a dataset for supervised machine learning after extracting patters from them. Finally the temporal logic formulas that were extracted are added to the pool of properties to be monitored, and the process restarts. They applied their approach to a subset of the CMAPSS dataset. Their approach can output temporal logic formulas as a way of explaining the RUL that is associated with the output. 
    \item XAI
    \item probabilistic Batesian generative model
    \item CMAPSS
    \item linear temporal logic and Symbolic Aggregate approXimation (SAX)
    \item none
    \item none
\end{itemize}

\cite{jang2019anomaly}
\begin{itemize}
    \item The authors develop an anomaly detection model for a 2.4L diesel engine. To simplify the problem, they focus on specifically two faults. The perform feature extraction with a variational autoencoder, and they using an One-Class Support Vector Machine (OCSVM) to distinguish between normal and anomalous states. They apply LIME to their OCSVM for explainability. 
    \item XAI
    \item AE for feature selection, One Class Support Vector Machine (OCSVM) for anomaly detection
    \item 2.4L diesel engine
    \item LIME
    \item accuracy, recall, precision
    \item none
\end{itemize}

\cite{cao2020using}
\begin{itemize}
    \item The authors create an approach based on knowledge-based systems for anomaly prediction. Their method is broken into 3 parts: pruning of chronicle rule base, integration of expert rules, and predictive maintenance. Pruning of chronicle rule base consists of mining the rules with frequent chronicle mining, translating the rules into SWRL rules, and best-quality rules selecting using accuracy (how many true rules) and coverage (how many true encompassing rules). The integration of expert rules involves receiving input from the experts and putting their rules to the same restrictions as the mined rules. Finally, the rules are used for anomaly prediction. They apply their system to semiconductors, and they showed they were able to achieve a good accuracy. 
    \item iML
    \item knowledge based system
    \item UCI SECOM, semiconductor manufactoring
    \item SWRL rules and ontologies
    \item average fitness value of first pareto front
    \item none, some rules come from experts
\end{itemize}

\cite{xu2021deep}
\begin{itemize}
    \item The authors are not only interested in anomaly detection, but also anomaly precursor detection. Anomaly precursors represent early symptoms of an upcoming anomaly. They argue that detecting precursors is useful for early prediction of anomalies to better understand when and what kind of anomaly will occur. They propose Multi-instance Contrastive learning approach with Dual Attention (MCDA) to tackle the problem of anomaly precursor detection. MCDA combines multi-instance learning and tensorized LSTM with time-dependent correlation to learn the precursors. A dual-attention module produces their interpretable results. They show that their method produces high accuracy results, and their attention mechanism provides variables which are explanatory for the results, which are verified by domain experts. 
    \item iML
    \item Multi-instance Contrastive learning approach with Dual Attention (MCDA) 
    \item refrigerators
    \item attention
    \item accuracy and f1
    \item verification with domain experts
\end{itemize}

\cite{ming2019interpretable}
\begin{itemize}
    \item The authors use the concept of prototype learning to construct a deep learning model with built-in interpretability. They introduce prototype sequence network (ProSeNet) for multi-class classification, in our interest fault diagnosis via diagnostic trouble codes. The model consists of a sequence encoder that is based on a recurrent architecture. The hidden state is fed into a prototype layer that determines how similar the hidden state is to prototypes in the form of a similarity vector. The network then outputs a prediction probability for the different classes based on the similarity vector. Interpretability can be conceived via the prototypes that are most similar to the input. They justified the interpretability of their model by using Amazon MTurk and surveying the users about the interpretability. They also studied how the input of human knowledge would affect the interpretability. They showed that including the human feedback improved the interpretability of their network in a post-study of different Amazon MTurk users. 
    \item iML
    \item ProSeNet - LSTM based encoder with prototype layer without multi-class classification
    \item Vehicle faults
    \item Prototype
    \item Recall and MAP
    \item utilizing Amazon MTurk, they were able to test and update their explainability via user input. Simplicity, diversity, and sparsity
\end{itemize}

\cite{yang2022noise}
\begin{itemize}
    \item The authors introduce the Noise-Aware Sparse Gaussian Process as a way of solving the scalability and noise sensitivity issues of normal Guassian Processes. Based on their NASGP algorithm, they develop an interpretable GAM that uses additive kernels and individual features. They apply their method to IEEE PHM 2012 data challenge in forms of RUL prediction and fault diagnosis. Their method performed well in comparison to other methods and allowed a level of interpretability.  
    \item iml
    \item Noise-Aware Sparse Gausian Process (NASGP) based GAM, generalized additive model
    \item PRONOSTIA platform and provided by the IEEE PHM 2012 Data Challenge 
    
    \item score, mae, nrmse
    \item They can match the coefficients to FFT which means that their method is able to capture the same information as FFT. This would make the case that it is in some realm interpretable.
\end{itemize}

\cite{steurtewagen2021adding}
\begin{itemize}
    \item The authors create a framework for fault diagnosis that consists of three parts: data collection, prognosis, and diagnosis. Importantly, in the data collection phase, they receive the reports that associate to the faults. The prognosis section uses an XGBoost algorithm to detect a fault occurring. The diagnosis utilizes SHAP to determine the features that are important to the output of XGBoost. These features are validated using the reports that accompany the fault. Notably, this would not be applicable to normal performing data.
    \item XAI
    \item XGBoost
    \item gas compressor units
    \item SHAP
    \item AUC
    \item they only performed evaluation to one feature, but they do compare the explanations with the accompanying reports
\end{itemize}

\cite{keleko2023health}
\begin{itemize}
    \item The authors propose a framework for fault diagnosis. First they develop a driven module that consits of a DNN for multi-class classification. Their second module aims to explain the first module via an explainable method, in this instance deepSHAP. They show good performance on multiple metrics for different faults. 
    \item XAI
    \item DNN Classifier
    \item Hydraulic systems
    \item DeepSHAP
    \item accuracy, f1, precision, recall
    \item none
\end{itemize}

\cite{costa2022variational}
\begin{itemize}
    \item The authors propose a new method for evaluating aircraft engine degradation. To overcome explainability of typical data-driven approaches, they propose a recurrent variational encoder for its ability to capture temporal dependencies and map the input data to a latent space. They argue the visualization of the latent space adds interpretability of the model by showing that an input maps to RULs that are similar within the latent space. They are able to achieve an interpretable latent space by ignoring a decoder and regularizing the latent space through variational inference
    \item iML
    \item Recurrent VAE
    \item CMAPSS
    \item visualizing latent representations
    \item Score function, RMSE
    \item none really, the engines with similar RULS are grouped together in the latent representation
\end{itemize}

\cite{kothamasu2007adaptive}
\begin{itemize}
    \item The authors present a Mamdani neuro-fuzzy modeling approach for two use cases, bearing fault detection and aircraft engine fault diagnosis. They chose this model as it has the following characteristics: adaptive, flexible, lucid, and robust. Their model consists of 5 layers: input, linguistic term input, rules, linguistic terms output, and defuzzification. The linguistic term layers translates the previous input into terms for the Mamdani rules via fuzzy membership functions. The rule layer only receives inputs from linguistic terms that are in the fuzzy rule. Finally the defuzzifaction layer receives input from the last linguistic term layer that correspond to that output parameter. As the rules can become undistinguisable through training, they utilize Kullback-Leibler mean information to refine the rules. 
    \item iML
    \item Adaptive Mamdani fuzzy model (AMFM)
    \item bearing and aircraft engines
    \item inherent interpretability via IF-THEN fuzzy rules
    \item accuracy
    \item none
\end{itemize}

\cite{salido2004comparison}
\begin{itemize}
    \item The authors create a fuzzy diagnosis system based on knowledge-based networks (KBN) and genetic algorithms (GA). The KBN constructs fuzzy rules using neural learning where the input is the features and the following layers are OR neurons and AND neurons. To determine the optimal number of neurons, they use GA. Importantly in their GA, they add a metric to measure simplicity of their rules by making more concise rules. With their architecture, they can 1) detect a fault and 2) explain the fault using an IF-THEN rule which can be used as a method of root cause analysis. 
    \item iML
    \item knowledge-based network
    \item transmission system of a pump
    \item extracted rules
    \item accuracy 
    \item simplicity of extracted rules
\end{itemize}

\cite{chen2020temporal}
\begin{itemize}
    \item Inspired by imitation learning, the authors performed fault diagnosis on a furnace using internet-of-things, reinforcement learning, and signal temporal logic. Their algorithm takes in the STL grammar and labeled input data, and it outputs an optimal STL formula. The agent chooses a formula from the agenda and adds it to a chart based on the current policy. The evaluator evaluates the performance of the formula on the input. The learner updates the policy function according to the performance. The agenda is updated based on the formulas in the chart. They utilize an MDP to construct the agenda-based formulas while the reinforcement learning solves the problem. The apply their method to multiple faults, and they show good robustness results, fast runtimes, and statistically significant performances.
    \item iML
    \item Reinforcement learning solving a MDP
    \item iron-making furnace
    \item Siganl temporal logic
    \item robustness, time, statistical test
    \item none
\end{itemize}

\cite{felsberger2020explainable}
\begin{itemize}
    \item The authors present a use-case where they apply XAI to a particle accelerator. They test a number of machine learning models including popular ones like kNN and RF. They found that the CNN based models that were tested performed the best overall, and they used LRP to show that the CNN based architectures were able to learn relevant features. The other architectures really established much of the possible features as relevant which led to low performance. 
    \item XAI
    \item FCN, FCN2drop, FCN3drop, tCNN, kNN, RF, SVM
    \item particle accelerator
    \item LRP
    \item accuracy and f1
    \item explanations verified by domain experts
\end{itemize}

\cite{matzka2020explainable}
\begin{itemize}
    \item The author performs 2 separate experiments: 1) measuring performance and feature importance of bagged tree ensemble and 2) training and analyzing multiple decision trees for evaluating explanatory performance. The bagged tree ensemble and the individual decision trees showed similar feature importance; this would insinuate that those features were actually more important than the others. 
    \item both
    \item Bagged tree ensemble, decision trees with specific inputs
    \item machine failure
    \item estimated predictor importance
    \item accuracy
    \item none
\end{itemize}

\cite{torcianti2021explainable}
\begin{itemize}
    \item This work is the future work of \cite{matzka2020explainable}. They utilize RUS boosted trees coupled with LIME to predict machine failure. After achieving a high accuracy with their model, they tested their LIME implementation. They normalized the relative feature importance values and set an importance threshold. They then rand LIME for selected datapoints and notes the imporance scores. They found that LIME would regularly report features that showed high importance. 
    \item XAI
    \item RUS boosted trees
    \item machine failure
    \item LIME
    \item accuracy
    \item scoring if the explanation included the essential features
\end{itemize}

\cite{sayed2022explainable}
\begin{itemize}
    \item The authors propose a framework for RUL estimation and decision-making support for the CMAPSS dataset. Their framework consists of 1) data preperation and analysis, 2) fault prognositcs and RUL estimation, and 3) decision-making support and explanation. 1) Discriminant features were selected using prognosability and trendability. Prognosability determines how well defined the end-of-life threshold is. Trendability measures the correlation between a feature and the time. 2) RUL estimation, while not the focus, was done via a random forest model. 3) Decision-making support and explanation consists of: 1) an explanation database created using SHAP, 2) an optimization engine that finds the most suitable maintenance actions with respect to a failure mode and estimated RUL, and 3) a human-machine interface that provides the explanation of maintenance actions at different forms and detail levels according to the user. They did not show the interface used. 
    \item XAI
    \item random forest
    \item CMAPSS
    \item SHAP
    \item r2 and rmse
    \item none
\end{itemize}

\cite{serradilla2020interpreting}
\begin{itemize}
    \item The authors perform remaining useful life prediction of a bushings testbed. They test 6 different models (Gaussian Naive Bayes, Linear Support Vector  Regressor,  K-Neighbors  Regressor,  Linear  Discriminant Analysis, Random Forest Regressor (final) and XGBoost Regressor) to determine which is better for their use case. They determine RFR was the best. They then utilize two explainability methods (ELI5 and LIME) to show global and local feature importance. Their main lesson is that these methods should be used to create more interpretable models in the future. 
    \item XAI
    \item Gaussian Naive Bayes, Linear Support Vector  Regressor,  K-Neighbors  Regressor,  Linear  Discriminant Analysis, Random Forest Regressor (final) and XGBoost Regressor
    \item Bushings
    \item ELI5(global) and LIME(local)
    \item Mean  Absolute  Error  (MAE)  and  Root  Mean  Square  Error (RMSE).
    \item none
\end{itemize}

\cite{khan2022explainable}
\begin{itemize}
    \item The authors combine a number of regression models with LIME and SHAP. They use the CMAPSS dataset as a benchmark to test their different models. Their MLP regressor outperformed the other models.
    \item XAI
    \item random forest, elasticnet with generalized linear models, gradient boosting, svms, nns
    \item CMAPSS 2008
    \item LIME and SHAP
    \item MSE and MAE
    \item None
\end{itemize}

\cite{upasane2021big}
\begin{itemize}
    \item The authors propose a type 2 fuzzy logic system for fault prediction to allow interpretability. They also utilize the Big-Bang Big-Crunch algorithm for optimization of their fuzzy logic system. Type 2 fuzzy logic is similar to type 1 fuzzy logic (normal fuzzy), but it comes with an uncertainty measurement. BB-BC is a heuristic population-based evolutionary algorithm that is used to optimize the number of antecedents in the fuzzy rules by minimizing RMSE. 
    \item iML
    \item Fuzzy sets, and fuzzy rules
    \item  two transducers (all sensors are transducers), one measures pressure, one measures current.
    \item fuzzy system
    \item RMSE 0.091
    \item none
\end{itemize}

\cite{jakubowski2022roll}
\begin{itemize}
    \item This work develops a predictive maintenance solution for an industrial cold rolling operation. They develop a semi-supervised algorithm based on the PIAE. Their algorithm is physics informed due to them appending phsyics information, from a list of equations that they provide, into the input data of their AE. Their model is more accurate than a base AE, and they provide explanations in the form of counterfactuals. 
    \item xai
    \item Physics infromed autoencoder (PIAE).
    \item cold-rolling operation
    \item Counterfactuals and physics constraints.
    \item Reconstruction error
    \item none
\end{itemize}


\cite{xu2022physics}
\begin{itemize}
    \item The authors propose the physics-constraint variational neural network (PCVNN) as applied to external gear pumps. The PCVNN is an asymmetric autoencoder. The encoder is a stacked CNN, BiLSTM, Attention network while the decoder is a generative physical model. This would allow for NN to learn the data, and it would allow the physical model to represent the learned patterns in a way that is consistent with the physics of the problem.
    \item iml
    \item CNN-LSTM-Attention and Physics Generative model
    \item Real data, harvested from a physical pump
    \item none (features are mapped to physics)
    \item Reconstruction error
    \item They can match the coefficients to FFT which means that their method is able to capture the same information as FFT. This would make the case that it is in some realm interpretable.
\end{itemize}

\cite{bellini2021deep}
\begin{itemize}
    \item The authors aim to model the maintenance events of a chemical plant. They model the faults as any subsection of the plant having a maintenance event. They model this using a CNN-LSTM with SHAP as an XAI method. 
    \item xai
    \item CNN-LSTM
    \item ALTAIR chemical plan
    \item SHAP 
    \item Precision, Recall, and F1 
    \item none
\end{itemize}

\cite{csalodi2021mixture}
\begin{itemize}
    \item The authors use a purely statistical model that breaks up a larger survival problem into smaller ones. The entities surviving (or not) are clustered based on how their variable values (multi-variate data was used, and feature selection was too) relate to their survival (thus it isn't that similarly variabled entities are clustered, similar relationships are clustered. Each cluster gets it own local model based on the Weibull distribution.
    \item iml
    \item statistical model, gaussian mixture model, fuzzy clustering
    \item lithium-ion batteries
    \item none (just statistics)
    \item none
    \item none
\end{itemize}

\cite{Remil2021-kr}
\begin{itemize}
    \item fault diagnosis
    \item XAI
    \item SplitSD4X
\end{itemize}

\cite{Ding2021-ez}
\begin{itemize}
    \item prognosis
    \item iml
\end{itemize}


\cite{Zhang2021-ee}
\begin{itemize}
    \item detection
    \item xai
\end{itemize}

\cite{Mahmoodian2022-zk}
\begin{itemize}
    \item iml
    \item diagnosis
\end{itemize}

\cite{Kononov2023-ys}
\begin{itemize}
    \item xai
    \item prognosis
\end{itemize}

\cite{Ghasemkhani2023-rd}
\begin{itemize}
    \item detection
    \item xai
\end{itemize}

\cite{Solis-Martin2023-po}
\begin{itemize}
    \item xai
    \item prognosis
\end{itemize}

\cite{Alfeo2022-or}
\begin{itemize}
    \item xai
    \item prognosis
\end{itemize}

\cite{Allah_Bukhsh2019-bk}
\begin{itemize}
    \item xai
    \item detection
\end{itemize}

\cite{Xia2023-bg}
\begin{itemize}
    \item iml
    \item diagnosis
\end{itemize}

\cite{Amram2021-gt}
\begin{itemize}
    \item prognosis
    \item iml
\end{itemize}

\cite{Wang2023-px}
\begin{itemize}
    \item prognosis
    \item xai
\end{itemize}

\cite{Tod2023-cf}
\begin{itemize}
    \item prognosis
    \item iml
\end{itemize}



\cite{Simmons2021-hj}
\begin{itemize}
    \item prognosis
    \item xai
\end{itemize}

\cite{voronov2021forest}
\begin{itemize}
    \item iml
    \item prognosis
\end{itemize}

\cite{konovalenko2022generating}
\begin{itemize}
    \item iml
    \item detection
\end{itemize}

\cite{manco2017fault}
\begin{itemize}
    \item xai
    \item detection
\end{itemize}

\cite{Protopapadakis2022-ye}
\begin{itemize}
    \item xai
    \item prognosis
\end{itemize}



\cite{Abbas2022-mm}
\begin{itemize}
    \item prognosis
    \item iml
\end{itemize}

\cite{Beretta2021-gk}
\begin{itemize}
    \item detection
    \item iml
\end{itemize}

\cite{Han2022-yk}
\begin{itemize}
    \item xai
    \item diagnosis
\end{itemize}

\cite{Jakubowski2022-hh}
\begin{itemize}
    \item xai
    \item prognosis
\end{itemize}

\cite{Li2021-ri}
\begin{itemize}
    \item xai
    \item detection
\end{itemize}

\cite{Ferraro2023-jv}
\begin{itemize}
    \item xai 
    \item prognosis
\end{itemize}

\cite{Upasane2023-al}
\begin{itemize}
    \item detection
    \item iml
\end{itemize}


\cite{Jing2022-yq}
\begin{itemize}
    \item prognosis
    \item iml
\end{itemize}

\cite{Castle2020-pc}
\begin{itemize}
    \item prognosis
    \item iml 
\end{itemize}

\cite{Waghen2022-na}
\begin{itemize}
    \item iml
    \item prognosis
\end{itemize}

\cite{Hajgato2022-ia}
\begin{itemize}
    \item xai
    \item detection
\end{itemize}

\cite{Bakdi2022-gw}
\begin{itemize}
    \item xai
    \item prognosis
\end{itemize}

\cite{Schmetz2021-pf}
\begin{itemize}
    \item detection
    \item xai
\end{itemize}

\cite{Dhaou2021-qx}
\begin{itemize}
    \item detection
    \item iml 
\end{itemize}
